Efficient Optimal Transport Algorithm by Accelerated Gradient descent

Optimal transport (OT) plays an essential role in various areas like machine learning and deep learning. However, computing discrete optimal transport plan for large scale problems with adequate accuracy and efficiency is still highly challenging. Recently, methods based on the Sinkhorn algorithm add an entropy regularizer to the prime problem and get a trade off between efficiency and accuracy. In this paper, we propose a novel algorithm to further improve the efficiency and accuracy based on Nesterov's smoothing technique. Basically, the non-smooth c-transform of the Kantorovich potential is approximated by the smooth Log-Sum-Exp function, which finally smooths the original non-smooth Kantorovich dual functional (energy). The smooth Kantorovich functional can be optimized by the fast proximal gradient algorithm (FISTA) efficiently. Theoretically, the computational complexity of the proposed method is given by $O(n^{\frac{5}{2}} \sqrt{\log n} /\epsilon)$, which is lower than that of the Sinkhorn algorithm. Empirically, compared with the Sinkhorn algorithm, our experimental results demonstrate that the proposed method achieves faster convergence and better accuracy with the same parameter.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> related_work.tex <==
\vspace{-3mm}
\section{Related Work}
Optimal transport plays an important role in various kinds of fields, and there is a huge literature in this area. Here we'll mainly focus on the most related works. For detailed overview, we refer the readers to \cite{peyre2018COT}.
% and \cite{solomon2018OTDD}.

% For the semi-discrete optimal transport problem, where the source density function is absolutely continuous and the target measure is discrete, Aurenhammer et. al \cite{Aurenhammer1998Minkowski} and Gu et.al \cite{gu2013theory} give geometric variational approaches to solve it with squared Euclidean distance cost. Kitagawa et. al extended their methods in \cite{Kitagawa2019otnewton} for general source distribution and cost functions. Under the above settings, the Kantorovich functional is smooth and strictly convex, and thus can be optimized by Newton's method.

When both the source and target measures are discrete, the OT problem can be treated as a standard linear programming (LP) task and can be solved by interior-point method with computational complexity $\tilde{O}(n^{5/2})$ \cite{Lee2014LP}. But this method requires a practical solver of the Laplacian linear system, which is not available currently for large dataset. Another interior-point based method to solve the OT problem is proposed by Pele and Werman \cite{Pele2009EM} with complexity $\tilde{O}(n^3)$. Generally speaking, it is unrealistic to solve the large scale OT problem with the traditional LP solvers.

The prevalent way to compute the OT distance between two discrete measures involves adding the strongly convex entropy function into the prime Kantorovich problem \cite{Cuturi2013Sinkhorn, Benamou2015sinkhorn}. Most of the current solutions for the discrete OT problem follow this strategy. Genevay et al. \cite{genevay2016stochastic} extend the algorithm in its dual form and solve it by stochastic average gradient method.
The Greenkhorn algorithm~ \cite{Altschuler2017greenhorn, Abid2018greedygreenhorn, Chakrabarty2018greenhorn} is a greedy version of the Sinkhorn algorithm. Specifically, Altschuler et al. \cite{Altschuler2017greenhorn} show that the complexity of their algorithm is $\tilde{O}(\frac{n^2}{\epsilon^3})$. Later, Dvurechensky et al. \cite{Dvurechensky2018PD} improve the complexity bound of the Sinkhorn algorithm to $\tilde{O}(\frac{n^2}{\epsilon^2})$, and propose an adaptive primal-dual accelerated gradient descent (APDAGD) method with complexity $\tilde{O}(\min \{\frac{n^{9/4}}{\epsilon}, \frac{n^2}{\epsilon^2}\})$. Jambulapati et al. \cite{Jambulapati2019parallel} introduce a parallelelizable algorithm to compute the OT problem with complexity $\tilde{O}(\frac{n^2\|C\|_{\max}}{\epsilon})$.
Through screening the negligible components by directly setting them at that value before entering the Sinkhorn problem, the screenkhorn \cite{Alaya2019screenhorn} method solves a smaller Sinkhorn problem and improve the computation efficiency.
Based on a primal-dual formulation and a tight upper bound for the dual solution, Lin et al. \cite{Lin2019(APDAMD} improve the complexity bound of the Greenkhorn algorithm to $\tilde{O}(\frac{n^2}{\epsilon^2})$, and propose the adaptive primal-dual accelerated mirror descent(APDAMD) algorithm, whose complexity bound is proven to be $\tilde{O}(\frac{n^2 \sqrt{r}}{\epsilon})$, where $r\in(0,n]$ refers  to some constants in the Bregman divergence. 
Recently, a more practically efficient method called APDRCD \cite{Guo2020APDRCD} is proposed with complexity $\tilde{O}(n^{2.5}/\epsilon)$. But all these three primal-dual based methods need to build a matrix with space complexity $O(n^3)$, which makes them impractical when $n$ is large.
% With hybrid algorithm to initialize the Sinkhorn/Greenhorn, Lin et al. \cite{Lin2019accSinkhorn} establish the complexity bounds of $\tilde{O}(\frac{n^{7/3}}{\epsilon})$. 
By utilizing Newton-type information, Blanchet et al. \cite{Blanchet2020Hessian} and Quanrud \cite{Quanrud2018Hessian} propose algorithms with complexity $\tilde{O}(\frac{n^2}{\epsilon})$. However, the Newton-based methods are complex and have no available code currently.

Besides the entropy regularizer based methods, Blondel et al. \cite{Blondel2018sot} use the squared 2-norm and group lasso to regularize the prime Kantorovich problem and then use the quasi-Newton method to accelerate the algorithm. Xie et al. \cite{Xie2019proximal} develop an Inexact Proximal point method for exact optimal transport. By utilizing the structure of the cost function, Gerber and Maggioni \cite{Gerber2017multiscale} optimize the transport plan from coarse to fine.
Meng et.al \cite{meng2019ppmm} propose the projection pursuit Monge map, which accelerates the computation of the original sliced OT problem.  Xie et al. \cite{xie2019ipot} also use the generative learning based method to model the optimal transport. But the theoretical analysis of these algorithms is still nascent.

In this work, we introduce a method based on Nesterov's smoothing technique, which is applied to the dual Kantorovich problem with computational complexity $O(n^{2.5}\sqrt{\log~ n}/\varepsilon)$ (or equivalently $\tilde{O}(n^{2.5}/\varepsilon)$) and approximation error bound $2\lambda \log n$.

==> supp_experiments.tex <==
\section{More Experiments}
In this section, we firstly show the convergent curves of $E_\lambda(\psi)$, $\langle P_\lambda, C \rangle$ and $E(\psi)$ with the metrics of squared Euclidean distance and spherical distance. Then we test the performance of the proposed algorithm under different cost functions to show that $E(\psi_\lambda)$ provides a better approximation than $\langle P_\lambda, C \rangle$ by the Sinkhorn algorithm \cite{Cuturi2013Sinkhorn}.

\begin{figure*}[]
\centering
\begin{tabular}{cc}
    \includegraphics[width=.45\linewidth]{figure/supp/supp_SED.png} &
    \includegraphics[width=.45\linewidth]{figure/supp/supp_SD.png}
\end{tabular}
\vspace{-3mm}
\caption{The convergent curves of $E(\psi)$, $E_\lambda(\psi)$ and $\langle P_\lambda, C\rangle$.}
    \label{fig:curves}
\end{figure*}

\begin{table*}[t]
\centering
\caption{Comparison among the OT cost (GT), the Sinkhorn result and the result of the proposed method with $T=500$ under different $P$.}
\label{tab:P_compare}
\begin{tabular}{c|ccc|cc}
\hline
P   & GT      & Sinkhorn & Ours    & |Sinkhorn-GT| & |Ours-GT| \\ \hline
1.5 & 103.33  & 103.51   & 103.27  & 0.18          & \textbf{0.06}      \\ \hline
2   & 281.7   & 282.5    & 281.6   & 0.8           & \textbf{0.1}       \\ \hline
3   & 2189.8  & 2197.1   & 2187.5  & 7.3           & \textbf{2.3}       \\ \hline
4   & 16951.4 & 17038.5  & 16932.0 & 87.1          & \textbf{19.4}      \\ \hline
\end{tabular}
\end{table*}

\subsection{More illustrations of $T$ and $\eta$}
\textbf{The Parameter $T$} The computer can only represent numbers in fixed precision. For example, if double-precision floating-point format is used in 64-bit processors, the range of the number is about $2.2251e^{-308} \sim 1.7977e^{+308}$ when using MATLAB. Based on the property 1 of the problem (\ref{eq:cpt2}), the optimal solvers of $E(\psi)$ with respect to the original cost matrix $C$ and the new matrix $C-\frac{\max(C)+\min(C)}{2}$ are the same. Thus,
to fully utilize the range of the exponential for current computer architecture and get more accurate results, we  set $C=C-\frac{\max(C)+\min(C)}{2}$. If taking no consideration of $\psi$, $\lambda$ can be as small as about $\frac{R}{600}$ in Eqn. (\ref{eqn: smooth_energy}) to keep numerical stability, namely no 'Inf' or 'NAN' output. In reality, we set $\lambda = \frac{R}{T}$ and use $T$ to control $\lambda$. Here $R=\max(C)-\min(C)$. Larger $T$ will give better approximation.

\textbf{The Parameter $\eta$} For the FISTA algorithm, the ideal fixed step size is $\eta_t=\frac{1}{\lambda_{\max}}$, where $\lambda_{\max}$ is the maximum eigenvalue of the Hessian matrix, as shown in Eqn. (\ref{eqn:Hessian}). However, accurate estimate of $\lambda_{\max}$ is hard and we only know $\lambda_{\max} \leq \frac{1}{\lambda}$, so we turn to set $\eta_t = \eta \lambda$. For one thing, if $\lambda$ is relatively large, only with small step size, the algorithm may run out of the precision range of the processor and thus get 'Inf' or 'NAN'. Thus, $\eta$ may be far less that $1$. For the other thing, we have $H\leq \frac{1}{\lambda}\max_i(\frac{\max_j K_{ij}v_j}{\mathbf{K_iv}})\leq \frac{1}{\lambda}$, we may also choose $\eta > 1$ when $\lambda$ itself is small. As a result, for different tasks, $\eta$ may change a lot. 


\subsection{More experimental results}
In this experiment, we set $m=n=500$, $T=500$, and adjust $\eta$ to get the best performance of the proposed algorithm. Basically, for the squared Euclidean distance, $\eta=50$; for the spherical distance, $\eta=0.02$. In Fig. \ref{fig:curves}, we show the performance of $E(\psi)$, $E_\lambda(\psi)$ and $\langle P_\lambda, C\rangle$, where $P_\lambda$ is the approximate transport plan computed by Eqn. (\ref{eq:ot_plan}) with parameter $\lambda$. It is obvious that when the algorithm converges, we have $\langle P_\lambda^*, C\rangle \geq \langle P^*, C\rangle = - E(\psi^*) \geq - E(\psi_\lambda^*)$. Here $P_\lambda^*$ is the computed approximate OT plan given the optimizer $\psi_\lambda^*$ for $E_\lambda(\psi)$, $P^*$ and $\psi^*$ are the OT plan and optimal solver for $E(\psi)$, respectively. Though both $\langle P_\lambda^*, C\rangle$ and $-E(\psi_\lambda^*)$ approximate the optimal transport cost well, the latter performs much better.


We also explore this phenomenon with more experiments. We randomly sample $m=500$ samples from the Gaussian distribution $\mathcal{N}(3\mathbf{1}_5, \mathbf{I}_5)$ as the support of the source measure, represented by $x_i, i=1,2,\ldots,m$; and randomly sample $n=500$ samples from the Uniform distribution $Uni([-5,-4]^5)$ as the support of the target measure, denoted by $y_j,j=1,2,\ldots,n$. The source and target measures are given by $\mu=\sum_{i=1}^m \mu_i\delta(x-x_i)$ and $\nu=\sum_{j=1}^n \nu_i\delta(y-y_i)$, where both $\mu_i$s and $\nu_j$s are sampled from the uniform distribution $Uni([0,1])$ and then normalized by $\mu_i=\mu_i/\sum_{i=1}^m \mu_i$ and $\nu_j=\nu_j/\sum_{j=1}^n \nu_i$. The cost function is set as $c(x_i, y_j)=\|x_i-y_j\|^P$ with $P=1.5,2,3,4$, respectively. In Tab. \ref{tab:P_compare}, we show the OT cost given by linear programming, the Sinkhorn result and $-E(\psi_\lambda^*)$ by setting $T=500$. It is obvious that as $P$ increase, the error of the Sinkhorn result and the proposed method also increase. However, our results performs much better than Sinkhorn. This matches our analysis that Sinkhorn requires much smaller $\lambda$ to get the same error bound $\epsilon$.
Moreover, if we set $T=800$, which means that we use a much smaller $\lambda$, the proposed method still works and gets more accurate results, while the Sinkhorn will return 'NAN' due to numerical overflow. It's interesting to investigate the relationship between approximate accuracy and cost functions, and we leave this part for the future work.
% \subsection{Large scale dataset}
% It is hard to get the groundtruth transport cost for large scale problems, so here we choose to densely sample from two Gaussian distributions, namely $\mu = N(\mathbf{m}_1, \Sigma_1)$ and $\nu=N(\mathbf{m}_2, \Sigma_2)$. The 2-Wasserstein distance between $\mu$ and $\nu$ is given by 
% \[
% W_2(\mu, \nu)^2 = \|m_1-m_2\|^2 + trace(\Sigma_1+\Sigma_2 - 2(\Sigma_2^{1/2}\Sigma_1\Sigma_2^{1/2})^{1/2})
% \]
% In the following experiment,we set $\mathbf{m}_1 = (-5.0,0.0)^T, \Sigma_1 = I$ and $\mathbf{m}_2 = (0.0,5.0)^T, \Sigma_2 = I$, then the 2-Wasserstein distance between $\mu$ and $\nu$ is 50. Next, we densely sample $10000$ samples from both $\mu$ and $\nu$, and the samples are denoted by $x_i$s and $y_j$s. The discrete distributions $\hat{\mu} = \frac{1}{10000}\sum_{i=1}^{10000}\delta(x-x_i)$ and $\hat{\nu} = \frac{1}{10000}\sum_{j=1}^{10000} \delta(y-y_j)$ can be used to approximate $\mu$ and $\nu$, respectively. Thus, we compute the transport cost or 2-Wasserstein distance between $\hat{\mu}$ and $\hat{\nu}$. We set $T=500$ for both our algorithm and the sinkhorn algorithm \cite{Cuturi2013Sinkhorn}, and adjust $\eta$ to get the best performance. We show the results in Fig. \ref{fig:large_scale}. From the figure we can see that though our algorithm converges a little slower than the sinkhorn algorithm under the squared Euclidean distance, the approximate accuracy of our method is better.

% \begin{figure*}[t]
% \centering
% \begin{tabular}{cc}
%     \includegraphics[width=.45\linewidth]{figure/supp/10000_SED.png} &
%     \includegraphics[width=.45\linewidth]{figure/supp/10000_SED_L1.png}
    
% \end{tabular}
% \vspace{-3mm}
% \caption{The performance of the proposed algorithm with large scale dataset.}
%     \label{fig:large_scale}
%     \vspace{-2mm}
% \end{figure*}
